A baseline revisited: Pushing the limits of multi-segment models for context-aware translation

This paper addresses the task of contextual translation using multi-segment models. Specifically we show that increasing model capacity further pushes the limits of this approach and that deeper models are more suited to capture context dependencies. Furthermore, improvements observed with larger models can be transferred to smaller models using knowledge distillation. Our experiments show that this approach achieves competitive performance across several languages and benchmarks, without additional language-specific tuning and task specific architectures.

==> extra.tex <==

\subsection{Document level monolingual data for distillation}

%Data sparsity has been succesfully addressed in prior work by backtranslation or forward translation using different flavours teacher models (Facebook paper). In this work we present the first results with forward translation of source original monolingual data using a teacher model and distillation to a shallow model. We not that prior work showed that back-translation data has been overestimated due to evaluation done on testsets where the source segments are translationeese (translations into that langauge) rather than fluent segments in the source language. Results in Table\ref{ForwardTranslationMonolingual}

While results on accuracy for targeted test sets in table \ref{tab:large_small_distill} shows improvement for all student models, one can argue that for some of them there is still a significant gap compare to the teachers performance and that there is room for improvement. We found that we can partially address this issue by using the teacher model to do forward-translation on documents level monolingual text and add it as training data for the student model. Improvement for the student model using monolingual data can be observed in table \ref{tab:large_small_distill}.


\begin{table}[h]
\centering
%\resizebox{\textwidth}{!}{
%\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\hline
 & \textbf{WMT} & \multicolumn{2}{c}{\textbf{ContraPro}} \\
 &  \textbf{BLEU} & \multicolumn{2}{c}{\textbf{Accuracy}}\\
\textbf{Model} &  \textbf{w/ ctx} & \textbf{w/ ctx} & \textbf{w/o ctx}\\
\hline
 D-6x6 & 30.6 & 0.77 & 0.51\\
 ST-6x2 & 31.1 & 0.73 & 0.49\\
 \ + augment& 31.3 & 0.75 & 0.49\\
\hline
\end{tabular}
%}
\caption{Results for EN-DE on training data augmentation with forward translated document-level monolingual data. \label{ForwardTranslationMonolingual}}
\label{tab:large_small_distill}
\end{table}


%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{Figures/ForwardTranslationMonolingual}
%\end{center}
%\caption{Training data augmentation with forward translated document-level monolingual data. \label{ForwardTranslationMonolingual}}
%\end{figure}



\subsection{Ablation by length}

We observe a large degradation in performance for test sentences with a length that is four standard deviations away from the average training data length. Similar performance degradation has been examined in prior work, suggesting that positional embeddings for the longer sentences are not seen enough during training. In our work we observe that while all models degrade, the student model performance better than the teacher model. We hypothesis that the student model performs better because it suffers less from exposure bias and error propagation, as it is trained on data coming from the teacher model distribution which is simpler and therefore easier to learn as well as more similar to the inference time behaviour.

\cite{nguyen-etal-2021-data} investigate the behaviour of models trained on large contexts and observe improvements due to length diversity, and (to a lesser extent) position shifting. This suggests that with data augmentation by concatenation of random sentences we may solve the issue with degradation while keeping the improvements from useful discourse information.  

%* Data Augmentation by Concatenation for Low-Resource Translation: A Mystery and a Solution * 

%The paper explores the BLEU gains for low resource languages by concatenating random sentences. Comparing BLEU scores of concatenation of random sentences vs consecutive sentences in a document they conclude that gains do not come from document context. Through several experiments they find that the gains come from three aspects: 1. adding random sentences helps the model learn what NOT to attend to, 2. concatenation leads to longer sentences which in term helps translate long sentences because otherwise large positional embeddings are rarely seen in training, 3. a diversity in sentence length for batches that concatenation leads to (although the last point isn’t described very clearly in the paper). One of the points made in the paper is that absolute positional embeddings don’t allow for generalizing well to longer sequences in a low resource setting. Therefore, it would be interesting to see how relative positional embeddings compare.

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{Figures/AblationSegmentLength2}
\end{center}
\caption{Segment length analysis. \label{AblationSegmentLength}}

\end{figure*}

\subsection{Ablation by context type}

\paragraph{Context conditions} We contrast translation quality measures of a model when translating data in context versus translating the same segments in isolation. We add a third condition, by translating segments when paired with random context. We introduce this as a measure of contextual models robustness. Contextual models should be able to discriminate between relevant and irrelevant context and not degrade quality in the latter case. We apply the same three conditions for both generic and targeted metrics. We introduce the following notation (\gd{or maybe move this to a table}) (\gd{it would be good to show that without this third measurement we have models that are very non-robust}). :
\begin{itemize}
    \item Metric$_{\mathrm{NoCtx}}$, $_{\mathrm{PreCtx}}$, $_{\mathrm{RndCtx}}$ where the three conditions stand for \textit{no context}, \textit{preceding context} and \textit{random context}.
    \item Generic quality metrics: one of BLUE or XX
    \item Targeted quality metrics: Anaphora accuracy (\gd{define and give example or add examples a table}) Deixis accuracy
\end{itemize}

We investigate if the model is able to distinguish between relevant context or noisy context. We look at the performance measured by BLEU on the generic testset and accuracy on the targeted testset. We observe that providing random context degrades performance on the discourse phenomena testset, indicating the model is trying to resolve the sentence level ambiguity (pronoun translation) by looking at contextual information, however it expects the context to be relevant. On the generic testset, we observe that with random context the performance is slightly improved, indicating that for generic sentences without discourse phenomena the model learns to disregard irelevant context. 

\paragraph{Context sensitivity}
In order to quantify how context-sensitive models are, irrespective of the quality, we propose two measures of \textit{context sensitivity}. We compare models w.r.t. their context sensitivity by measuring the difference between the translation in context and  translation in isolation, where difference is the inverse of any similarity metric (such as BLEU, ChrF). Formally, we define $\mathrm{CS}$ (context sensitivity) as: 
\begin{itemize}
    \item $\mathrm{CS}_{\mathrm{PreCtx}} = 1-\mathrm{ChrF}(T_{\mathrm{PreCtx}}, T_{\mathrm{NoCtx}})$ where $T_{\mathrm{PreCtx}}$ and $T_{\mathrm{NoCtx}}$ are translations using the preceding context and no context, respectively.
    \item Similarly, $\mathrm{CS}_{\mathrm{RndCtx}}$ measures the difference between translation in isolation and translation in random context. 
\end{itemize}



\begin{table*}[t]
\centering
%\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccc}
\hline
 &  \multicolumn{3}{c}{\textbf{WMT - BLEU}} &  \multicolumn{3}{c}{\textbf{ContraPro - Accuracy}} \\
 \textbf{Model} & \textbf{w/ ctx} &  \textbf{w/o ctx} &  \textbf{rand ctx} & \textbf{w/ ctx} & \textbf{w/o ctx} & \textbf{rand ctx}\\
\hline
S-6x2 & 29.4 & 30.1 & 29.9 & 0.7 & 0.51 & 0.37\\
D-6x6 & 30.6 & 31.3 & 30.9 & 0.77 & 0.51 & 0.37\\
ST-6x2 & 31.1 & 32.1 & 31.6 & 0.73 & 0.49 & 0.36\\
\hline
\end{tabular}
%}
\caption{Performance of contextual model with random context on EN-DE. \label{AblationRandomContext}}
\end{table*}



\section{Notes}
\gd{Depth vs width results
\begin{itemize}
    \item Any other previous work comparing depth vs width in translation models. Anything that confirms our findings? We also have depth/width results internally on WinoMT (pronoun resolution needed, but within sentence).
    \item Analysis of what is going on: is it context usage overall that differs, is it "good" context usage? e.g. use the context usage metrics or brainstorm for other way to get insight.
    \item Do a human eval to try and qualify the differences between deeper/wider. 
    \item In pronouns tests, is anything else qualitatively different in depth/width other than pronouns?
\end{itemize}
}

\gd{More generally: how is this work different from addressing translation of long sentences (and review previous work on segment length). e.g. this of 2 inputs of the same length, one multi-segment and one single-segment. What are the differences/similarities, which one do we want to improve on? (Particularly relevant because of the 2+2 method used, which does not actually distinguish, modeling-wise, between multi or single-segment input.)}

%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{Figures/AblationRandomContext}
%\end{center}
%\caption{Performance of contextual model with random context. \label{AblationRandomContext}}
%\end{figure}

%\subsection{Data sparsity}
%Data sparsity has been succesfully addressed in prior work by backtranslation or forward translation using different flavours teacher models (Facebook paper). In this work we present the first results with forward translation of source original monolingual data using a teacher model and distillation to a shallow model. We not that prior work showed that back-translation data has been overestimated due to evaluation done on testsets where the source segments are translationeese (translations into that langauge) rather than fluent segments in the source language. Results in Table\ref{ForwardTranslationMonolingual}



%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=0.8\textwidth]{Figures/ForwardTranslationMonolingual}
%\end{center}
%\caption{Training data augmentation with forward translated document-level monolingual data.}
%\label{ForwardTranslationMonolingual}
%\end{figure}



%\begin{table*}[t]
%\centering
%\begin{tabular}{llcccccc}
%\hline
%& &  \multicolumn{2}{c}{{WMT/IWSLT}} &  \multicolumn{4}{c}{{Targeted test set (See Table XX)}}\\
%{LP} &  {Model} & {BLEU$_{\mathrm{Ctx}}$} & {BLEU$_{\mathrm{NoCtx}}$} & {BLEU$_{\mathrm{Ctx}}$} & {BLEU$_{\mathrm{NoCtx}}$}&  {Acc$_{\mathrm{Ctx}}$} & {Acc$_{\mathrm{NoCtx}}$} \\
%\hline
%EN-DE & Base & -& 29.9 & - & 19.9 & - & 0.49\\
%     & 2+2 & 29.4& \textbf{30.1} & 21.8 & \textbf{20.2} & 0.70 & 0.51\\
%\hline
%EN-FR & Base & -&  41.8 & - & 31.9 & - & 0.50\\
%      & 2+2 & 41.7& ? & 33.7 & 32.7 & 0.73 & 0.50\\
%\hline
%EN-RU & Base & -& 14.7 & - & - & - & 0.50 \\
%     & 2+2 & 15.5 & ? & - & - & 0.82 & 0.50\\
%\end{tabular}
%\caption{\gd{To remove the numbers in bold - they complicate the narative, introduce them only in length ablation experiment} Comparison of context no context - S-6x2  models - slide 15 from Suvodeep}
%\label{tab:context_no_context}
%\end{table*}


%\begin{tabular}{l|c|ccccccc}
%\hline
%           &  &    &    & \multicolumn{4}{c}{Dist. to disambiguating ctx (\% of total data)} \\
%{Model} & NewsT/SelAtt Bleu & Bleu & Acc-Total & 0 (20\%) & 1(59\%) & 2(12\%) & 3(5\%) & >3(4\%)\\
%\hline
% Base-44M  & 29.9 & 19.9  & 0.49 & 0.74 & 0.39 & 0.47 & 0.49 & 0.62\\
% Base-Deep-60M  & 30.9 & 20.3 & 0.51 & 0.81 & 0.41 & 0.48 & 0.52 & 0.64\\
% 44M       & 29.4 & 21.8  & 0.70 & 0.77 & 0.70 & 0.62 & 0.62 & 0.76\\
% \hline
% Deep-52M   & & \gd{22.2} & 0.75 & 0.81 & 0.75 & 0.67 & 0.67 & 0.81 \\
% Deep-60M  & 30.6 & 22.5  & 0.77 & 0.82 & 0.77 & 0.68 & 0.70 & 0.77\\
% Deep-60M-mask  & 31.1 & ?  & 0.77 & 0.83 & 0.77 & 0.68 & 0.68 & 0.80\\
% Deep-68M   &  /\gd{32.0} & \gd{22.9}  & 0.78 & 0.82 & 0.79 & 0.68 & 0.66 & 0.77\\
% Deep-76M   & & \gd{22.4}  & 0.74 & 0.79 & 0.74 & 0.69 & 0.69 & 0.76 \\
% \hline
% Wide-52M   & & \gd{22.2}  & ? & ? & ? & ? & ? &\\
% Wide-60M  & & 22.2 & 0.73 & ? & ? & ? & ? &\\
% Wide-68M   & & \gd{22.3}  & 0.73 & 0.79 & 0.74 & 0.62 & 0.64 & 0.78\\
% Wide-76M   & & \gd{22.5} & 0.73 & 0.78 & 0.73 & 0.64 & 0.64 & 0.76\\     
%      \hline 
% \cite{lopes-etal-2020-document} \footnote{Table 7. concat is the best, but not in all tasks (see table 6).}  &  &  & 0.71 & ? & ? & ? & ? & \\
% \cite{fernandes21acl} 2to2\footnote{+dropout, trained on 200k IWSLT}& & ? & 0.66 & ? & ? & ? & ? & \\
% \cite{fernandes21acl} 2to2+pre\footnote{+dropout, trained on 200k IWSLT + 82mil monolingual}& ? & & 0.80 & ? & ? & ? & ? & \\  
% \cite{maruf-etal-2019-selective}-offline\footnote{54M params. Tables 4 and 5} & & ? & ? & 0.69 & 0.35 & 0.46 & 0.51 & 0.68\\
% \cite{maruf-etal-2019-selective}-online & ? & & ? & 0.73 & 0.34 & 0.46 & 0.48 & 0.66\\
%\end{tabular}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

